Points2Plans: From Point Clouds to Long-Horizon Plans with Composable Relational Dynamics

We present Points2Plans, a framework for composable planning with a relational dynamics model that enables robots to solve long-horizon manipulation tasks from partial-view point clouds. Given a language instruction and a point cloud of the scene, our framework initiates a hierarchical planning procedure, whereby a language model generates a high-level plan and a sampling-based planner produces constraint-satisfying continuous parameters for manipulation primitives sequenced according to the high-level plan. Key to our approach is the use of a relational dynamics model as a unifying interface between the continuous and symbolic representations of states and actions, thus facilitating language-driven planning from high-dimensional perceptual input such as point clouds. Whereas previous relational dynamics models require training on datasets of multi-step manipulation scenarios that align with the intended test scenarios, Points2Plans uses only single-step simulated training data while generalizing zero-shot to a variable number of steps during real-world evaluations. We evaluate our approach on tasks involving geometric reasoning, multi-object interactions, and occluded object reasoning in both simulated and real-world settings. Results demonstrate that Points2Plans offers strong generalization to unseen long-horizon tasks in the real world, where it solves over 85% of evaluated tasks while the next best baseline solves only 50%.

==> overview_fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
  \begin{center}
    \centering
    \includegraphics[width=\textwidth]{figures/figure_1_v12.pdf}
    \vspace{-20pt}
  \end{center}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:overview_figure}}~\textbf{Training, planning, and execution phases of \cp{}.}  \textbf{Left:} In simulation, we sample an environment state and execute a manipulation primitive at random to generate a dataset of single-step environment transitions and train a relational dynamics model. \textbf{Middle:} At planning time, \cp{} receives a language instruction and a partial-view, segmented point cloud of the scene and then performs long-horizon planning in a hierarchical fashion with a task planner (e.g., a language model) and the learned relational dynamics model. If planning is successful, \cp{} returns a sequence of manipulation primitives (what to execute) and their associated continuous parameters (how to execute them) for the given task. \textbf{Right:} \cp{} executes its plan to solve a variety of unseen long-horizon tasks in the real world.}
  \vspace{-18pt}
  \medskip}
\makeatother
\shrinka
\maketitle
\shrinka
\thispagestyle{empty}
\pagestyle{empty}
